Visual Foresight: Model-Based Deep Reinforcement Learning for Vision-Based Robotic Control

Deep reinforcement learning (RL) algorithms can learn complex robotic skills from raw sensory inputs, but have yet to achieve the kind of broad generalization and applicability demonstrated by deep learning methods in supervised domains. We present a deep RL method that is practical for real-world robotics tasks, such as robotic manipulation, and generalizes effectively to never-before-seen tasks and objects. In these settings, ground truth reward signals are typically unavailable, and we therefore propose a self-supervised model-based approach, where a predictive model learns to directly predict the future from raw sensory readings, such as camera images. At test time, we explore three distinct goal specification methods: designated pixels, where a user specifies desired object manipulation tasks by selecting particular pixels in an image and corresponding goal positions, goal images, where the desired goal state is specified with an image, and image classifiers, which define spaces of goal states. Our deep predictive models are trained using data collected autonomously and continuously by a robot interacting with hundreds of objects, without human supervision. We demonstrate that visual MPC can generalize to never-before-seen objects---both rigid and deformable---and solve a range of user-defined object manipulation tasks using the same model.

==> cost_functions.tex <==
\section{Planning Cost Functions}
\label{sec:cost}

In this section, we discuss how to specify and evaluate goals for planning. One na\"{i}ve approach is to use pixel-wise error, such as $\ell_2$ error, between a \emph{goal image} and the \emph{predicted image}. However there is a severe issue with this approach: large objects in the image, i.e. the arm and shadows, dominate such a cost; therefore a common failure mode occurs when the planner matches the arm position with its position in the goal image, disregarding smaller objects. This failure motivates our use of more sophisticated mechanisms for specifying goals, which we discuss next.

\subsection{Pixel Distance Cost}
\label{subsec:pixel_dist_cost}
A convenient way to define a robot task is by choosing one or more \emph{designated pixels} in the robot's camera view and choosing a destination where each pixel should be moved. For example, the user might select a pixel on an object and ask the robot to move it 10 cm to the left. This type of objective is general, in that it can define any object relocation task on the viewing plane. Further, success can be measured quantitatively, as detailed in section \ref{sec:experiments}.
Given a distribution over pixel positions $P_0$, our model predicts distributions over its positions $P_t$ at time $t \in \{ 1, \dots, T \}$. One way of defining the cost per time-step $c_t$ is by using the expected Euclidean distance to the goal point $d_g$, which is straight-forward to calculate from $P_t$ and $g$, as follows:
 \begin{align}
c = \sum_{t = 1, \dots, T} c_t =  \sum_{t = 1, \dots, T} \mathbb{E}_{\hat{d}_{t} \sim P_{t}} \left[\|\hat{d}_{t} - d_{g}\|_2\right] 
 \label{eq:cost}
 \end{align}
The per time-step costs $c_t$ are summed together giving the overall planing objective $c$. The expected distance to the goal provides a smooth planning objective and enables longer-horizon tasks, since this cost function encourages movement of the designated objects into the right direction for each step of the execution, regardless of whether the goal-position can be reached within $T$ time steps or not. This cost also makes use of the uncertainty estimates of the predictor when computing the expected distance to the goal. For multi-objective tasks with multiple designated pixels $d^{(i)}$ the costs are summed to together, and optionally weighted according to a scheme discussed in \autoref{subsec:reg_cost}.  

\subsection{Registration-Based Cost}
\label{subsec:reg_cost}
We now propose an improvement over using pixel distances. When using pixel distance cost functions, it is necessary to know the \emph{current} location of the object,  $\pixel_0^{(1)}, \dots, \pixel_0^{(P)}$ at each replanning step, so that the model can predict the positions of this pixel from the current step forward.
To update the belief of where the target object currently is, we propose to register the current image to the start and optionally also to a \emph{goal image}, where the designated pixels are marked by the user. Adding a goal image can make visual MPC more precise, since when the target object is close to the goal position, registration to the goal-image greatly improves the position estimate of the designated pixel. Crucially, the registration method we introduce is self-supervised, using the same exact data for training the video prediction model and for training the registration model. This allows both models to continuously improve as the robot collects more data.

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{images_rfr/registration_singletime.pdf}
	\vspace{-0.3cm}
	\caption{\small{Closed loop control is achieved by registering the current image $I_t$ globally to the first frame $I_0$ and the goal image $I_g$. In this example registration to $I_0$ succeeds while registration to $I_g$ fails since the object in $I_g$ is too far away.}
		\label{fig:reg_single}
	}
\end{figure}

\noindent \textbf{Test time procedure.}
We will first describe the registration scheme at test time (see Figure~\ref{fig:registration_arch}(a)). We separately register the current image $I_t$ to the start image $I_0$ and to the goal image $I_g$ by passing it into the registration network $R$, implemented as a fully-convolutional neural network. The registration network produces a flow map $\hat{F}_{0 \leftarrow t} \in \mathbb{R}^{H \times W \times 2}$, a vector field with the same size as the image, that describes the relative motion for every pixel between the two frames.
\begin{align}
\hat{F}_{0 \leftarrow t} = R(I_t, I_0) &&
\hat{F}_{g \leftarrow t} = R(I_t, I_g)
\end{align}
The flow map $\hat{F}_{0 \leftarrow t}$ can be used to warp the image of the current time step $t$ to the start image $I_0$, and $\hat{F}_{g \leftarrow t}$ can be used to warp from $I_t$ to $I_g$ (see Figure \ref{fig:reg_single} for an illustration). There is no difference to the warping operation used in the video prediction model, explained in section \ref{sec:model}, equation \ref{simple_dna}:
\begin{align}
\hat{I}_0 = \hat{F}_{0 \leftarrow t} \diamond  I_t &&
\hat{I}_g = \hat{F}_{g \leftarrow t} \diamond  I_t 
\end{align}
In essence for a current image $\hat{F}_{0 \leftarrow t}$ puts $I_t$ in correspondence with $I_0$, and $\hat{F}_{g \leftarrow t}$ puts $I_t$ in correspondence with $I_g$. The motivation for registering to both $I_0$ and $I_g$ is to increase accuracy and robustness. In principle, registering to either $I_0$ or $I_g$ is sufficient.
While the registration network is trained to perform a global registration between the images, we only evaluate it at the points $d_0$ and $d_g$ chosen by the user. This results in a cost function that ignores distractors. The flow map produced by the registration network is used to find the pixel locations corresponding to $d_0$ and $d_g$ in the current frame: 
\begin{align}
\hat{d}_{0,t} = d_0 + \hat{F}_{0 \leftarrow t}(d_0) &&
\hat{d}_{g,t} = d_g + \hat{F}_{g \leftarrow t}(d_g)
\label{eqn:warped_pos}
\end{align}


\begin{figure}[t!]
	\centering
	\begin{subfigure}[b]{0.35\linewidth}
		\centering
		\includegraphics[width=\linewidth]{images_rfr/registration_test_start.pdf}\vspace{2.5mm}
		\includegraphics[width=\linewidth]{images_rfr/registration_test_goal.pdf}
		\caption{\small{Testing usage.}}
	\end{subfigure}
	\quad \quad
	\begin{subfigure}[b]{0.55\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim={0 3mm 0 3mm},clip]{images_rfr/registration_train.pdf}
		\caption{\small{Training usage.}}
		\label{fig:discrete}
	\end{subfigure}
	\vspace{-1mm}
	\caption{\small{(a) At test time the registration network registers the current image $I_t$ to the start image $I_0$ (top) and goal image $I_g$ (bottom), inferring the flow-fields $\hat{F}_{0 \leftarrow t}$ and $\hat{F}_{g \leftarrow t}$. (b) The registration network is trained by warping images from randomly selected timesteps along a trajectory to each other.
	}}
	\label{fig:registration_arch}
\end{figure}

\begin{figure*}
	\centering
	\vspace{-0.1in}	\includegraphics[width=1\linewidth]{images_rfr/reg_over_time.png}
	\caption{\small{Outputs of registration network. The first row shows the timesteps from left to right of a robot picking and moving a red bowl, the second row shows each image warped to the initial image via registration, and the third row shows the same for the goal image. A successful registration in this visualization would result in images that closely resemble the start- or goal image. In the first row, the locations where the designated pixel of the start image $d_0$ and the goal image $d_g$ are found are marked with red and blue crosses, respectively. It can be seen that the registration to the start image (red cross) is failing in the second to last time step, while the registration to the goal image (blue cross) succeeds for all time steps. The numbers in red, in the upper left corners indicate the trade off factors $\lambda$ between the views and are used as weighting factors for the planning cost. (Best viewed in PDF)}}
	\label{fig:tracking_overtime}
	\vspace{-0.2in}
\end{figure*}

For simplicity, we describe the case with a single designated pixel. In practice, instead of a single flow vector $\hat{F}_{0 \leftarrow t}(d_0)$ and $\hat{F}_{g \leftarrow t}(d_g)$, we consider a neighborhood of flow-vectors around $d_0$ and $d_g$ and take the median in the $x$ and $y$ directions, making the registration more stable.
\autoref{fig:tracking_overtime} visualizes an example tracking result while the gripper is moving an object.

\noindent \textbf{Registration-based pixel distance cost.}
Registration can fail when distances between objects in the images are large. During a motion, the registration to the first image typically becomes harder, while the registration to the goal image becomes easier. We propose a mechanism that estimates which image is registered correctly, allowing us to utilize only the successful registration for evaluating the planning cost. This mechanism gives a high weight $\lambda_i$ to pixel distance costs $c_i$ associated with a designated pixel $\hat{d}_{i,t}$ that is tracked successfully and a low, ideally zero, weight to a designated pixel where the registration is poor. We use the photometric distance between the true frame and the warped frame evaluated at $d_{0,i}$ and $d_{g,i}$ as an estimate for \emph{local} registration success. A low photometric error indicates that the registration network predicted a flow vector leading to a pixel with a similar color, thus indicating warping success. However this does not necessarily mean that the flow vector points to the correct location. For example, there could be several objects with the same color and the network could simply point to the wrong object. Letting $I_i(d_i)$ denote the pixel value in image $I_i$ for position $d_i$, and $\hat{I}_i(d_i)$ denote the corresponding pixel in the image warped by the registration function, we can define the general weighting factors $\lambda_i$ as:
\begin{align}
\lambda_i =  \frac{||I_i(d_i) - \hat{I_i}(d_i)||_2^{-1}}{\sum^N_j ||I_j(d_j) - \hat{I}_j(d_j)||^{-1}_2}.
\label{eqn:cost_avg}
\end{align}
where $\hat{I}_i = \hat{F}_{i \leftarrow t} \diamond I_t$. The MPC cost is computed as the average of the costs $c_i$ weighted by $\lambda_i$, where each $c_i$ is the expected distance (see equation \ref{eq:cost}) between the registered point $\hat{d}_{i,t}$ and the goal point $d_{g,i}$. Hence, the cost used for planning is $c = \sum_i \lambda_i c_i$.  In the case of the single view model and a single designated pixel, the index $i$ iterates over the start and goal image (and $N=2$).

The proposed weighting scheme can also be used with multiple designated pixels, as used in multi-task settings and multi-view models, which are explained in section \ref{sec:multiview}. The index $i$ then also loops over the views and indices of the designated pixels.

\noindent \textbf{Training procedure.}
The registration network is trained on the same data as the video prediction model, but it does not share parameters with it.\footnote{In principle, sharing parameters with the video prediction model might be beneficial, but this is left for future work.} Our approach is similar to the optic flow method proposed by \cite{meister2017unflow}. However, unlike this prior work, our method computes registrations for frames that might be many time steps apart, and the goal is not to extract optic flow, but rather to determine correspondences between potentially distant images. For training, two images are sampled at random times steps $t$ and $t+h$ along the trajectory and the images are warped to each other in both directions. 
\begin{align}
\hat{I}_{t} = \hat{F}_{t \leftarrow t +h} \diamond  I_{t+h} &&
\hat{I}_{t+h} = \hat{F}_{t+h \leftarrow t} \diamond  I_{t}
\end{align}
The network, which outputs $\hat{F}_{t \leftarrow t +h}$ and $\hat{F}_{t+h \leftarrow t}$, see Figure~\ref{fig:registration_arch} (b), is trained to minimize the photometric distance between $\hat{I}_t$ and $I_t$ and $\hat{I}_{t+h}$ and $I_{t+h}$, in addition to a smoothness regularizer that penalizes abrupt changes in the outputted flow-field. The details of this loss function follow prior work \cite{meister2017unflow}. We found that gradually increasing the temporal distance $h$ between the images during training yielded better final accuracy, as it creates a learning curriculum. The temporal distance is linearly increased from 1 step to 8 steps at 20k SGD steps. In total 60k iterations were taken.

The network $R$ is implemented as a fully convolutional network taking in two images stacked along the channel dimension. First the inputs are passed into three convolutional layers each followed by a bilinear downsampling operation. This is passed into three layers of convolution each followed by a bilinear upsampling operation (all convolutions use stride 1). By using bilinear sampling for increasing or decreasing image sizes we avoid artifacts that are caused by strided convolutions and deconvolutions.


\subsection{Classifier-Based Cost Functions}
\label{subsec:class_cost}
An alternative way to define the cost function is with a goal classifier. This type of cost function is particularly well-suited for tasks that can be completed in multiple ways. For example, for a task of rearranging a pair objects into relative positions, i.e. pushing the first object to the left of the second object, the absolute positions of the objects do not matter nor does the arm position. A classifier-based cost function allows the planner to discover any of the possible goal states. 

Unfortunately, a typical image classifier will require a large amount of labeled examples to learn, and we do not want to collect large datasets for each and every task. Instead, we aim to learn a goal classifier from only a few positive examples, using a meta-learning approach. A few positive examples of success are easy for people to provide and are the minimal information needed to convey a goal.

\newcommand{\task}{\mathcal{T}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\obs}{\mathbf{o}}
\newcommand{\out}{y}
\newcommand{\posdata}{\data^+}
\newcommand{\testdata}{\data^\text{test}}
\newcommand{\loss}{\mathcal{L}}

Formally, we consider a goal classifier $\hat{\out} = f(\obs)$, where $\obs$ denotes the image observation, and $\hat{\out} \in [0,1]$ indicates the predicted probability of the observation being of a successful outcome of the task. Our objective is to infer a classifier for a new task $\task_j$ from a few positive examples of success, which are easy for a user to provide and encode the minimal information needed to convey a task. In other words, given a dataset $\posdata_j$ of $K$ examples of successful end states for a new task $\task_j$: $\data_j:=\{(\obs_k, 1) | k = 1...K\}_j$, our goal is to infer a classifier for task $\task_j$. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{images_cls/cls_fig_2.jpeg}
    \caption{\small We propose a framework for quickly specifying visual goals. Our goal classifier is meta-trained with positive and negative examples for diverse tasks (left), which allows it to meta-learn that some factors matter for goals (e.g., relative positions of objects), while some do not (e.g. position of the arm). At meta-test time, this classifier can learn goals for new tasks from a few of examples of success (right - the goal is to place the fork to the right of the plate). The cost can be derived from the learned goal classifier for use with visual MPC.}
    \label{fig:cls_fig}
    \vspace{-0.3cm}
\end{figure}

\noindent \textbf{Meta-learning for few-shot goal inference.}
To solve the above problem, we propose learning a few-shot classifier that can infer the goal of a new task from a small set of goal examples, allowing the user to define a task from a few examples of success. To train the few-shot classifier, we first collect a dataset of both positive and negative examples for a wide range of tasks. We then use this data to learn how to learn goal classifiers from a few positive examples.
Our approach is illustrated in Figure~\ref{fig:cls_fig}.

We build upon model-agnostic meta-learning (MAML)~\cite{maml}, which learns initial parameters $\theta$ for model $f$ that can efficiently adapt to a new task with one or a few steps of gradient descent. Grant et al. \cite{caml} proposed an extension of MAML, referred to as concept acquisition through meta-learning (CAML), for learning to learn new concepts from positive examples alone. We apply CAML to the setting of acquiring goal classifiers from positive examples, using a meta-training data with both positive and negative examples. The result of the meta-training procedure is an initial set of parameters that can be used to learn new goal classifiers at test time.

\noindent \textbf{Test time procedure.}
At test time, the user provides a dataset $\posdata_j$ of $K$ examples of successful end states for a new task $\task_j$: $\data_j:=\{(\obs_k, 1) | k = 1...K\}_j$, which are then used to infer a task-specific goal classifier $C_j$. In particular, the meta-learned parameters $\theta$ are updated through gradient descent to adapt to task $\task_j$:

$$
C_j(\obs)
= f(\obs; \theta_j')
= f\big(\obs; \theta-\alpha \nabla_\theta \!\!\! \sum_{(\obs_n, \out_n)\in \posdata_j} \loss (\out_n, f(\obs_n; \theta)\big)
$$

where $\loss$ is the cross-entropy loss function, $\alpha$ is the step size, and $\theta'$ denotes the parameters updated through gradient descent on task $\task_j$.

During planning, the learned classifier $C_j$ takes as input an image generated by the video prediction model and outputs the predicted probability of the goal being achieved for the task specified by the few examples of success. To convert this into a cost function, we treat the probability of success as the planning cost for that observation. To reduce the effect of false positives and mis-calibrated predictions, we use the classifier conservatively by thresholding the predictions so that reward is only given for confident successes. Below this threshold, we give a reward of 0 and above this threshold, we provide the predicted probability as the reward.


\noindent \textbf{Training time procedure.}
During meta-training, we explicitly train for the ability to infer goal classifiers for the set of training tasks, $\{ \task_i \}$. We assume a small dataset $\data_i$ for each task $\task_i$, consisting of both positive and negative examples: $\data_i:= \{(\obs_n,\out_n) | n=1...N \}_i$. To learn the initial parameters $\theta$, we optimize the following objective using Adam~\cite{ADAM}:

$$
\min_\theta \sum_i \sum_{(\obs_n, y_n) \in \testdata_i} \loss(\out_n, f(\obs_n; \theta_i')) 
$$

In our experiments, our classifier is represented by a convolutional neural network, consisting of three convolutional layers, each followed by layer normalization and a ReLU non-linearity. After the final convolutional layer, a spatial soft-argmax operation extracts spatial feature points, which are then passed through fully-connected layers.

\subsection{When to Use Which Cost Function?}
\label{subsec:cost_discuission}

We have introduced three different forms of cost function, pixel distance based cost functions with and without registration, as well as classifier-based cost functions. Here we discuss the relative strengths and weaknesses of each.

Pixel distance based cost functions have the advantage that they allow moving objects precisely to target locations. They are also easy to specify, without requiring any example goal images, and therefore provide an easy and fast user interface. The pixel distance based cost function also has a high degree of robustness against distractor objects and clutter, since the optimizer can ignore the values of other pixels; this is important when targeting diverse real-world environments.
By incorporating an image of the goal, we can also add a registration mechanism to allow for more robust closed-loop control, at the cost of a more significant burden on the user.

The classifier-based cost function allows for solving more abstract tasks since it can capture invariances, such as the position of the arm, and settings where the absolute positions of an object is not relevant, such as positioning a cup in front of a plate, irrespective of where the plate is.  Providing a few example images takes more effort than specifying pixel locations but allows a broader range of goal sets to be specified.



==> defs.tex <==
%% editing comment
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
\newcommand{\todo}[1]{\cmt{TO-DO: #1}}
\newcommand{\sergey}[1]{\cmt{Sergey: #1}}
\newcommand{\chelsea}[1]{\cmt{Chelsea: #1}}
\newcommand{\pieter}[1]{\cmt{Pieter: #1}}

%% ignore text
\long\def\ignorethis#1{}

%% abbreviations
\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% defines autoref commands
\def\sectionautorefname{Section}
\let\subsectionautorefname\sectionautorefname
\let\subsubsectionautorefname\sectionautorefname
\providecommand\algorithmname{Algorithm}
\def\equationautorefname~#1\null{Equation~(#1)\null}
\def\appendixautorefname{Appendix}

%% reference shortcuts
\newcommand{\figtodo}[1]{\framebox[0.8\columnwidth]{\rule{0pt}{1in}#1}}
\newcommand{\figref}[1]{\autoref{#1}}
%\renewcommand{\eqref}[1]{\autoref{#1}}
\newcommand{\secref}[1]{\autoref{#1}}

%% citation shortcuts
\newcommand{\atari}{acvpa-oglls-15}
\newcommand{\nyu}{vpbmse-mcl-16}

\newcommand{\model}{\mathcal{M}}
\newcommand{\action}{\mathbf{a}}
\newcommand{\state}{\mathbf{x}}
\newcommand{\image}{I_t}
\newcommand{\flow}{\hat{F}}
\newcommand{\pixel}{d} % the designated pixel
\newcommand{\pixelstate}{s} % the state of the desginated pixel
\newcommand{\goal}{g}




==> intro.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
  

Humans are faced with a stream of high-dimensional sensory inputs and minimal external supervision, and yet, are able to learn a range of complex, generalizable skills and behaviors.
While there has been significant progress in developing deep reinforcement learning algorithms that learn complex skills and scale to high-dimensional observation spaces, such as pixels~\cite{tdgammon,atari,e2e,alphago}, learning behaviors that \emph{generalize} to new tasks and objects remains an open problem.
The key to generalization is diversity. When deployed in a narrow, closed-world environment, a reinforcement learning algorithm will recover skills that are successful only in a narrow range of settings. 
Learning skills in diverse  environments, such as the real world, presents a number of significant challenges: external reward feedback is extremely sparse or non-existent, and the agent has only indirect access to the state of the world through its senses, which, in the case of a robot, might correspond to cameras and joint encoders.


We approach the problem of learning generalizable behavior in the real world from the standpoint of sensory prediction. Prediction is often considered a fundamental component of intelligence \cite{predictionandbrain}. Through prediction, it is possible to learn useful concepts about the world even from a raw stream of sensory observations, such as images from a camera. If we predict raw sensory observations directly, we do not need to assume availability of low-dimensional state information or an extrinsic reward signal.  Image observations are both information-rich and high-dimensional, presenting both an opportunity and a challenge. Future observations provide a substantial amount of supervisory information for a machine learning algorithm. However, the predictive model must have the capacity to predict these high-dimensional observations, and the control algorithm must be able to use such a model to effectively select actions to accomplish human-specified goals.  Examples of such goals are shown in figure \ref{fig:example_traj}.

We study control via prediction in the context of robotic manipulation, formulating a model-based reinforcement learning approach centered around prediction of raw sensory observations. One of the biggest challenges in learning-based robotic manipulation is generalization: how can we learn models that are useful not just for a narrow range of tasks seen during training, but that can be used to perform new tasks with new objects that were not seen previously?
Collecting a training dataset that is sufficiently rich and diverse is often challenging in highly-structured robotics experiments, which depend on human intervention for reward signals, resets, and safety constraints. We instead set up a minimally structured robotic control domain, where data is collected by the robot via unsupervised interaction with a wide range of objects, making it practical to collect large amounts of interaction data. The robot collects a stream of raw sensory observations (image pixels), without any reward signal at training time, and without the ability to reset the environment between episodes. This setting is both realistic and necessary for studying RL in diverse real-world environments, as it enables automated and unattended collection of diverse interaction experience. Since the training setting affords no readily accessible reward signal, learning by prediction presents an appealing option: the supervision signal for prediction is always available even in the stream of unsupervised experience.
We therefore propose to learn action-conditioned predictive models directly on raw pixel observations, and show that they can be used to accomplish a range of pixel-based manipulation tasks on a real robot in the physical world at test-time. 

%
%
%
%
%
%
%
%
%
%
The main contributions of this work are as follows. We present \emph{visual MPC}, a general framework for deep reinforcement learning with sensory prediction models that is suitable for learning behaviors in diverse, open-world environments (see figure~\ref{fig:overview}).
We describe deep neural network architectures that are effective for predicting pixel-level observations amid occlusions and with novel objects. Unlike low-dimensional representations of state, specifying and evaluating the reward from pixel predictions at test-time is nontrivial: we present several practical methods for specifying and evaluating progress towards the goal---including distances to goal pixel positions, registration to goal images, and success classifiers---and compare their effectiveness and use-cases.
%
%
Finally, our evaluation shows how these components can be combined to enable a real robot to perform a range of object manipulation tasks from raw pixel observations. Our experiments include manipulation of previously unseen objects, handling multiple objects, pushing objects around obstructions, handling clutter, manipulating deformable objects such as cloth, recovering from large perturbations, and grasping and maneuvering objects to user-specified locations in 3D-space. Our results represent a significant advance in the \emph{generality} of skills that can be acquired by a real robot operating on raw pixel values using a single model.

This article combines and extends material from several prior conference papers~\cite{foresight,sna,ebert2018robustness,flo}, presenting them in the context of a unified system. We include additional experiments, including cloth manipulation and placing tasks, a quantitative \emph{multi-task} experiment assessing the performance of our method on a wide range of distinct tasks with a single model, as well as a comprehensive, open-sourced simulation environment to facilitate future research and better reproducibility. The code and videos can be found on the project webpage\footnote{For videos \& code: \url{https://sites.google.com/view/visualforesight}}.
%
%

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth,trim={0mm 0 0 0},clip]{images_general/overview_roughdraft.png}
\caption{\small{Overview of visual MPC. (top) At training time, interaction data is collected autonomously and used to train a video-prediction model. (bottom) At test time, this model is used for sampling-based planning. In this work we discuss three different choices for the planning objective.}}
\label{fig:overview}
\end{figure}




 







==> optimizer.tex <==
\section{Trajectory Optimizer}

\begin{algorithm}[ht]
\caption{Planning in Visual MPC}
\label{alg:opt}
\begin{algorithmic}[1]
\State \textbf{Inputs:} Predictive model $g$, planning cost function $c$
\For{$t~=~0...T-1$}

\For{$i~=~0...n_{iter}-1$}
\If{$i==0$}
\State \begin{varwidth}[t]{\linewidth}
	Sample $M$ action sequences $\{a^{(m)}_{t:t+H-1}\}$ from \par $\mathcal N(0, I)$ or
	custom sampling distribution
\end{varwidth}
\Else
\State \begin{varwidth}[t]{\linewidth}
	Sample $M$ action sequences ${a^{(m)}_{t:t+H-1}}$ from \par 
	$\mathcal N(\mu^{(i)}, \Sigma^{(i)})$
\end{varwidth}
\EndIf
\State 
\begin{varwidth}[t]{\linewidth}
Check if sampled actions are within \par
admissible range, otherwise resample.
\end{varwidth}
\State  \begin{varwidth}[t]{\linewidth}
	Use $g$ to predict future  image sequences $\hat{I}_{t:t+H-1}^{(m)}$\\ and probability distributions $\hat{P}_{t:t+H-1}^{(m)}$
\end{varwidth}
\State Evaluate action sequences using a cost function $c$
\State  \begin{varwidth}[t]{\linewidth}
	Fit a diagonal Gaussian to the $k$  action samples\\ with lowest cost,
	yielding $\mu^{(i)}, \Sigma^{(i)}$
\end{varwidth}
\EndFor
\State Apply first action of best action sequence to robot
\EndFor
\end{algorithmic}
\end{algorithm}


\label{sec:optimizer}
The role of the optimizer is to find actions sequences $a_{1:T}$ that minimize the sum of the costs $c_{1:T}$ along the planning horizon $T$. We use a simple stochastic optimization procedure for this, based on the cross-entropy method (CEM), a gradient-free optimization procedure. CEM consists of iteratively resampling action sequences and refitting Gaussian distributions to the actions with the best predicted cost.

Although a variety of trajectory optimization methods may be suitable, one advantage of the stochastic optimization procedure is that it allows us to easily ensure that actions stay within the distribution of actions the model encountered during training. This is crucial to ensure that the model does not receive out-of-distribution inputs and makes valid predictions.  Algorithm \ref{alg:opt} illustrates the planning process. In practice this can be achieved by defining admissible ranges for each dimension of the action vector and rejecting a sample if it is outside of the admissible range. 

In the appendix \ref{sec:cem_improv} we present a few improvements to the CEM optimizer for visual MPC.
%


==> preliminaries.tex <==
\section{Overview}\label{sec:prelim}
\label{sec:vmpc}
%

%
In this section, we summarize our visual model-predictive control (MPC) method, which is a model-based reinforcement learning approach to end-to-end learning of robotic manipulation skills. Our method, outlined in Figure \ref{fig:overview}, consists of three phases: unsupervised data collection, predictive model training, and planning-based control via the model at test-time.

\noindent \textbf{Unsupervised data collection}: At \emph{training time}, data is collected autonomously by applying random actions sampled from a pre-specified distribution. It is important that this distribution allows the robot to visit parts of the state space that are relevant for solving the intended tasks. For some tasks, uniform random actions are sufficient, while for others, the design of the exploration strategy takes additional care, as detailed in Sections \ref{sec:system} and \ref{subsec:cloth_folding_data}.

\noindent \textbf{Model training}: Also during \emph{training time}, we train a video prediction model on the collected data. The model takes as input an image of the current timestep and a sequence of actions, and generates the corresponding sequence of future frames. This model is described in Section \ref{sec:model}.

\noindent \textbf{Test time control}: At \emph{test time}, we use a sampling-based, gradient free optimization procedure, similar to a shooting method~\cite{betts1998survey},
to find the sequence of actions that minimizes a cost function. Further details, including the motivation for this type of optimizer, can be found in Section \ref{sec:optimizer}. 

Depending on how the goal is specified, we use one of the following three cost functions. When the goal is provided by clicking on an object and a desired goal-position, a \emph{pixel-distance cost-function}, detailed in Section \ref{subsec:pixel_dist_cost}, evaluates how far the designated pixel is from the goal pixels. We can specify the goal more precisely by providing a goal image in addition to the pixel positions and make use of \emph{image-to-image registration} to compute a cost function, as discussed in Section \ref{subsec:reg_cost}. Finally, we show that we can specify more conceptual tasks
%
%
by providing one or several examples of success and employing a \emph{classifier-based} cost function as detailed in Section \ref{subsec:class_cost}. The strengths and weaknesses of different costs functions and trade-offs between them are discussed in Section \ref{subsec:cost_discuission}. 

The model is used to plan $T$ steps into the future, and the first action of the action sequence that attained lowest cost, is executed. In order to correct for mistakes made by the model, the actions are iteratively replanned at each real-world time step\footnote{With real-world step we mean timestep of the real-world as opposed to predicted timesteps.} $\tau \in \{0,...,\tau_{max}\}$ following the framework of model-predictive control (MPC). 
In the following sections, we explain the video-prediction model, the planning cost function, and the trajectory optimizer.


%








==> related_work.tex <==
\section{Related Work}\label{sec:rel_work}

%
%
%
%

\noindent \textbf{Model-based reinforcement learning.} Learning a model to predict the future, and then using this model to act, falls under the general umbrella of model-based reinforcement learning. Model-based RL algorithms are generally known to be more efficient than model-free methods~\cite{deisenroth2013survey}, and have been used with both low-dimensional~\cite{deisenroth2011pilco} and high-dimensional~\cite{deep_mpc} model classes. However, model-based RL methods that directly operate on raw image frames have not been studied as extensively. Several algorithms have been proposed for simple, synthetic images~\cite{watter2015embed} and video game environments~\cite{alexey, ha2018world, atarioh}, but have not been evaluated on generalization or in the real world, while other work has also studied model-based RL for individual robotic skills~\cite{dsae, zhang2018solar, se3}. In contrast to these works, we place special emphasis on \emph{generalization}, studying how predictive models can enable a real robot to manipulate previously unseen objects and solve new tasks.
Several prior works have also sought to learn inverse models that map from pairs of observations to actions, which can then be used greedily to carry out short-horizon tasks~\cite{agrawal2016learning,nair2017combining}. However, such methods do not directly construct longer-term plans, relying instead on greedy execution. In contrast, our method learns a forward model, which can be used to plan out a sequence of actions to achieve a user-specified goal.

%
%
%
%
%
%
%

\noindent \textbf{Self-supervised robotic learning.}
A number of recent works have studied self-supervised robotic learning, where large-scale unattended data collection is used to learn individual skills such as grasping~\cite{lerrel,google_handeye, calandra2017feeling,pinto2016curious}, push-grasp synergies~\cite{zeng2018learning}, or obstacle avoidance~\cite{greg_kahn_uncertainty,crashing}. 
In contrast to these methods, our approach learns predictive models that can be used to perform a variety of manipulation skills, and does not require a success measure, event indicator, or reward function during data collection.

\noindent \textbf{Sensory prediction models.}
We propose to leverage sensory prediction models, such as video-prediction models, to enable large-scale self-supervised learning of robotic skills. Prior work on action-conditioned video prediction has studied predicting synthetic video game images~\cite{atarioh,recurrentsimulators}, 3D point clouds~\cite{se3}, and real-world images~\cite{bootsetal,finn_nips,video_pixel_networks}, using both direct autoregressive frame prediction~\cite{beyond_mse,finn_nips,video_pixel_networks} and latent variable models~\cite{babaeizadeh2017stochastic,kurutach2018learning}. Several works have sought to use more complex distributions for future images, for example by using pixel autoregressive models~\cite{video_pixel_networks,scott_reed}. 
While this often produces sharp predictions, the resulting models are extremely demanding computationally.
Video prediction without actions has been studied for unstructured videos~\cite{beyond_mse,convlstm,vondrick} and driving~\cite{prednet,dynamic_filter_networks}.  In this work, we extend video prediction methods that are based on predicting a transformation from the previous image~\cite{finn_nips,dynamic_filter_networks}. 
%
%
%


==> scaling_up.tex <==
\section{Custom Action Sampling Distributions}

\label{sec:system}
When collecting data by sampling from simple distributions, such as a multivariate Gaussian, the skills that emerged were found to be generally restricted to pushing and dragging objects. This is because with simple distributions, it is very unlikely to visit states like picking up and placing of objects or folding cloth. Not only would the model be imprecise for these kinds of states, but also during planning it would be unlikely to \emph{find} action sequences that grasp an object or fold an item of clothing.
We therefore explore how the sampling distribution used both in data collection and sampling-based planning can be changed to visit these, otherwise unlikely, states more frequently, allowing more complex behavior to emerge. 

To allow picking up and placing of objects as well as folding of cloth to occur more frequently, we incorporate a simple ``reflex'' during data collection, where the gripper automatically closes, when the height of the wrist above the table is lower than a small threshold. This reflex is inspired by the palmar reflex observed in infants~\cite{grasping_fetal}. With this primitive, when collecting data with rigid objects about 20\% of trajectories included some sort of grasp. For deformable objects such as towels and cloth, this primitive helps increasing the likelihood of encountering states where cloths are folded. We found that the primitive can be slightly adapted to avoid cloths becoming tangled up. More details are provided in Appendix \ref{sec:folding_sampling}.

It is worth noting that, other than this reflex, no grasping-specific or folding-specific engineering was applied to the policy, allowing a joint pushing, grasping and folding policy to emerge through planning (see figure \ref{fig:push_grasp} in the appendix). In our experiments, we evaluate our method using data obtained both with and without the grasping reflex, evaluating both purely non-prehensile and combined prehensile and non-prehensile manipulation.

\section{Multi-View Visual MPC}
\label{sec:multiview}
\begin{wrapfigure}{r}{.5\columnwidth}
	\centering
	\includegraphics[width=0.5\columnwidth]{images_general/robot_setup_scheme.pdf}
	\caption{\small{Robot setup, with 2 standard web-cams arranged at different viewing angles.}}	\label{fig:robot_setup}
\end{wrapfigure}

The visual MPC algorithm as described so far is only able to solve manipulation tasks specified in 2D, like rearranging objects on the table. However, this can impose severe limitations; for example, a task such as lifting an object to a particular position in 3D cannot be fully specified with a single view, since it would be ambiguous. 
We use a combination of two views, taken from two cameras arranged appropriately, to jointly define a 3D task. Figure \ref{fig:robot_setup} shows the robot setup, including two standard webcams observing the workspace from different angles. The registration method described in the previous section is used separately per view to allow for dynamic retrying and solving temporally extended tasks. The planning costs from each view are combined using weighted averaging where the weights are provided by the registration network (see equation \ref{eqn:cost_avg}). Rows 5 and 6 of figure \ref{fig:tile_2} show a 3D object positioning task, where an object needs to be positioned at a particular point in 3D space. This task needs two views to be fully specified.







==> video_prediction.tex <==
\section{Video Prediction for Control}
\label{sec:model}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{images_general/prediction_model.pdf}
	\caption{\small{Computation graph of the video-prediction model. Time goes from left to right, $a_t$ are the actions, $h_t$ are the hidden states in the recurrent neural network, $\hat{F}_{t+1 \leftarrow t}$ is a 2D-warping field, $I_t$ are real images, and $\hat{I}_t$ are predicted images, $\mathcal{L}$ is a pairwise training-loss.}}   
	\label{fig:prediction_model}
\end{figure}

In visual MPC, we use a transformation-based video prediction architecture, first proposed by Finn et al. \cite{finn_nips}. The advantage of using transformation-based models over a model that directly generates pixels is two-fold: (1) prediction is easier, since the appearance of objects and the background scene can be reused from previous frames and (2) the transformations can be leveraged to obtain predictions about where pixels will move, a property that is used in several of our planning cost function formulations. The model, which is implemented as a recurrent neural network (RNN) $g_{\theta}$ parameterized by $\theta$, has a hidden state $h_t$ and takes in a previous image and an action at each step of the rollout.  Future images $\hat{I}_{t+1}$ are generated by warping the previous generated image $\hat{I}_t$ or the previous true image $I_t$, when available, according to a 2-dimensional flow field $\hat{F}_{t+1 \leftarrow t}$. A simplified illustration of model's structure is given in figure \ref{fig:prediction_model}. It is also summarized in the following two equations:
\begin{align}
[h_{t+1}, \hat{F}_{t+1 \leftarrow t}] 	&= g_{\theta}(a_t, h_t, I_t) \\
\hat{I}_{t+1} 							&= \hat{F}_{t+1 \leftarrow t} \diamond  \hat{I}_t 
\label{simple_dna}
\end{align}
Here, the bilinear sampling operator $\diamond$ interpolates the pixel values bilinearly with respect to a location $(x,y)$ and its four neighbouring pixels in the image, similar to \cite{zhou2016view}. Note that, as shown in figure \ref{fig:prediction_model}, at the first time-step the real image is transformed, whereas at later timesteps previously generated images are transformed in order to generate multi-frame predictions. The model is trained with gradient descent on a $\ell_2$ image reconstruction loss, denoted by $\mathcal{L}$ in figure \ref{fig:prediction_model}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images_sna/occlusionaware/architecture_2.pdf}
    \caption{\small{Forward pass through the recurrent SNA model. The red arrow indicates where the image from the first time step $I_0$ is concatenated with the transformed images $\hat{F}_{t+1 \leftarrow t} \diamond  \hat{I}_t $ multiplying each channel with a separate mask to produce the predicted frame for step $t+1$.}}      \label{fig:occlusion_model}
\end{figure}
A forward pass of the RNN is illustrated in figure \ref{fig:occlusion_model}. We use a series of stacked convolutional LSTMs and standard convolutional layers interleaved with average-pooling and upsampling layers. The result of this computation is the 2 dimensional flow-field $\hat{F}_{t+1 \leftarrow t}$ which is used to transform a current image $I_t$ or $\hat{I}_t$. More details on the architecture are provided in Appendix \ref{sec:skipcon}.

\noindent \textbf{Predicting pixel motion.} 
When using visual MPC with a cost-function based on start and goal pixel positions, we require a model that can effectively predict the 2D motion of the user-selected start pixels $\pixel_0^{(1)}, \dots, \pixel_0^{(P)}$ up to $T$ steps into the future\footnote{Note that when using a classifier-based cost function, we do not require the model to output transformations.}.
More details about the cost functions are provided in section \ref{sec:cost}. Since the model we employ is transformation-based, this motion prediction capability emerges automatically, and therefore no external pixel motion supervision is required. To predict the future positions of the designated pixel $d$, the same transformations used to transform the images are applied to the distribution over designated pixel locations. The warping transformation $\hat{F}_{t+1 \leftarrow t}$ can be interpreted as a stochastic transition operator allowing us to make probabilistic predictions about future locations of individual pixels:
\begin{equation}
\hat{P}_{t+1} = \hat{F}_{t+1 \leftarrow t} \diamond  \hat{P}_t
\label{eqn:prob_forward}
\end{equation}
Here, $P_t$ is a distribution over image locations which has the same spatial dimension as the image. For simplicity in notation, we will use a single designated pixel moving forward, but using multiple is straightforward. At the first time step, the distribution $\hat{P}_0$ is defined as 1 at the position of the user-selected designated pixel and zero elsewhere. The distribution $\hat{P}_{t+1}$ is normalized at each prediction step.

Since this basic model, referred to as dynamic neural advection (DNA), predicts images only based on the previous image, it is unable to recover shapes (e.g., objects) after they have been occluded, for example by the robot arm. Hence, this model is only suitable for planning motions where the user-selected pixels are not occluded during the manipulation, limiting its use in cluttered environments or with multiple selected pixels. In the next section, we introduce an enhanced model, which lifts this limitation by employing temporal skip connections. 

\noindent \textbf{Skip connection neural advection model.}
To enable effective tracking of objects through occlusions, we can add temporal skip connections to the model: we now transform pixels not only from the previously generated image $\hat{I}_t$, but from all previous images $\hat{I}_1,...\hat{I}_{t}$, including the context image $I_0$, which is a real image. All these transformed images can be combined to a form the predicted image $\hat{I}_{t+1}$ by taking a weighted sum over all transformed images, where the weights are given by masks $\mathbf{M}_t$ with the same size as the image and a single channel:
\begin{equation}
\hat{I}_{t+1} =  \mathbf{M}_{0} (\hat{F}_{t+1 \leftarrow 0} \diamond I_t) +  \sum_{j=1}^{\tau} \mathbf{M}_{j} (\hat{F}_{t+1 \leftarrow j} \diamond  \hat{I}_j).
\end{equation}
We refer to this model as the \emph{skip connection neural advection model (SNA)}, since it handles occlusions by using temporal skip connections such that when a pixel is occluded, e.g., by the robot arm or by another object, it can still reappear later in the sequence.
Transforming from all previous images comes with increased computational cost, since the number of masks and transformations scales with the number of time-steps $\tau$. However, we found that in practice a greatly simplified version of this model, where transformations are applied only to the previous image and the \emph{first image} of the sequence $I_0$, works equally well. Moreover we found that transforming the first image of the sequence is not necessary, as the model uses these pixels primarily to generate the image background. Therefore, we can use the first image directly, without transformation. More details can be found in the appendix \ref{sec:skipcon} and \cite{sna}.
